Nearly Optimal Communication and Query Complexity of Bipartite Matching

We settle the complexities of the maximum-cardinality bipartite matching problem (BMM) up to poly-logarithmic factors in five models of computation: the two-party communication, AND query, OR query, XOR query, and quantum edge query models. Our results answer open problems that have been raised repeatedly since at least three decades ago [Hajnal, Maass, and Turan STOC'88; Ivanyos, Klauck, Lee, Santha, and de Wolf FSTTCS'12; Dobzinski, Nisan, and Oren STOC'14; Nisan SODA'21] and tighten the lower bounds shown by Beniamini and Nisan [STOC'21] and Zhang [ICALP'04]. We also settle the communication complexity of the generalizations of BMM, such as maximum-cost bipartite $b$-matching and transshipment; and the query complexity of unique bipartite perfect matching (answering an open question by Beniamini [2022]). Our algorithms and lower bounds follow from simple applications of known techniques such as cutting planes methods and set disjointness.

==> cuttingplane.tex <==
\section{Alternatives to Center of Gravity}
\label{sec:cuttingplanes}
\jan{I feel this section might weaken our result as it makes it even more explicit that we "run just cutting planes". maybe it's better to just add a footnote in the proof that mentions instead of gravity center one could use analytic center as in \cite{Vaidya89}. To discuss.}

In \Cref{sec:BPM}, we described how to solve bipartite matching in various query complexity models by using the center of gravity based cutting plane method. 
Computing the center of gravity is NP-hard but there exist polynomial time alternatives.
For example, Vaidya's cutting plane method \cite{Vaidya89} uses the so called ``analytic center'' instead of the center of gravity, the former being computable in polynomial time via simple linear system solves.
%these alternatives are generaly more complicated which is why we used center of gravity in ref.

Here we outline that any $O(n\log n)$ iteration cutting plane method could be used to prove our results. 
The reduction is blackbox, so while it would prove our results, it does not give intuition of what the algorithm does and why it needs only $O(n \log n)$ iterations. %for why $O(n \log n)$ iterations suffice. 
This is why the proof in \Cref{sec:BPM} considers the center of gravity method as it allows for a short proof of why that variant of cutting planes converges in $O(n \log n)$ iterations.

The aim of cutting plane methods is to find a feasible point within some convex set. 
The crux is that this convex set is not explicitly given but only accessible via some ``separation oracle''.
This oracle can be given a point and then answers either ``feasible'' if the point is within the convex set, or returns a hyperplane separating the point from the feasible set.
Since the input is only accessed via this oracle, any cutting plane algorithm can be simulated in any query model by just implementing this oracle.
For example, in the 2-party model, each party can locally run exactly the same computations of the cutting plane method as long as both parties received the same separating hyperplanes from the oracle.
This also means that both parties locally compute the same point to be used for the next query to the oracle.
So it suffices to describe a communication protocol that, for some point known to both parties, computes a separating hyperplane or concludes the point is feasible.

\begin{lemma}\label{lem:2partoracle}
We can implement a separation oracle for \eqref{eq:MMF} in the 2-party model with $O(\log n)$ bits of communication.
\end{lemma}

\begin{proof}
The query point is known to both parties since it stems from previous local computations.
Each party just iterates over their set of edges and then sends a single $(u,v)$ with $p_u+p_v < 1$ if such an edge exists. The constraint $\{p_u+p_v \ge 1\}$ is then used as separating hyperplane.

If no such edge exists for either party, and $\sum_{v\in V}p_v \le F+1/3$ and $0\le p_v\le1$ for all $v$, then the point is feasible. Otherwise use the first of these constraints that was violated as separating hyperplane.
\end{proof}

\begin{lemma}\label{lem:ORoracle}
We can implement a separation oracle for \eqref{eq:MMF} in the OR-query model with $O(\log n)$ queries.
\end{lemma}

\begin{proof}
We binary search over all $u,v \in V$ pairs with $p_u + p_v < 1$ to find an edge $(u,v)$ with $p_u+p_v<1$.
Thus within $O(\log n)$ queries, we find a violating edge and can use $\{p_u+p_v\le1\}$ as separating hyperplane.

If no such edge exists, and $\sum_{v\in V}p_v \le F+1/3$ and $0\le p_v\le1$ for all $v$, then the point is feasible. Otherwise use the first of these constraints that was violated as separating hyperplane.
\end{proof}

We can use these separation oracles with any cutting plane method. The following algorithm by Vaidya \cite{Vaidya89} is deterministic, has a sufficiently small number of iterations, and does not compute NP-hard problems such as center of gravity.

\begin{lemma}[\cite{Vaidya89}]\label{lem:vaidya}
There exists the following deterministic cutting plane algorithm:
The input is a convex set represented via separation oracle, and a parameter $L>0$ such that the convex set is contained in a ball of radius $2^L$.
After $O(n L)$ calls to the oracle and $O(n^{\omega+1}L)$ additional time for other computations, the algorithm either finds a feasible point within the convex set, or concludes the convex set does not contain a ball of radius $2^{-L}$.
\end{lemma}

\Cref{lem:vaidya} together with the oracles from \Cref{lem:2partoracle,lem:ORoracle} 
and the volume bound \Cref{claim:volume_lower_bound}
imply that we can solve $BPM_n$ in $O(n \log^2 n)$ OR-queries and $O(n \log^2 n)$ bits of communication in the 2-party model.
The other models in \Cref{thm:BPM_in_all_models} follow from reductions in \Cref{sec:BPM}.

